Learning to Stop: Dynamic Simulation Monte-Carlo Tree Search

Monte Carlo tree search (MCTS) has achieved state-of-the-art results in many domains such as Go and Atari games when combining with deep neural networks (DNNs). When more simulations are executed, MCTS can achieve higher performance but also requires enormous amounts of CPU and GPU resources. However, not all states require a long searching time to identify the best action that the agent can find. For example, in 19x19 Go and NoGo, we found that for more than half of the states, the best action predicted by DNN remains unchanged even after searching 2 minutes. This implies that a significant amount of resources can be saved if we are able to stop the searching earlier when we are confident with the current searching result. In this paper, we propose to achieve this goal by predicting the uncertainty of the current searching status and use the result to decide whether we should stop searching. With our algorithm, called Dynamic Simulation MCTS (DS-MCTS), we can speed up a NoGo agent trained by AlphaZero 2.5 times faster while maintaining a similar winning rate. Also, under the same average simulation count, our method can achieve a 61% winning rate against the original program.

==> Figures/DifficultyExample.tex <==
\begin{figure}
    \centering
    \begin{subfigure} {0.3\textwidth}
        \centering
        \includegraphics[scale=0.25]{Figures/hard_state.PNG}
        \caption{Hard state.}
        \label{fig:hard_state}
    \end{subfigure}
    \begin{subfigure} {0.3\textwidth}
        \centering
        \includegraphics[scale=0.25]{Figures/easy_state.PNG}
        \caption{Easy state.}
        \label{fig:easy_state}
    \end{subfigure}
    \caption{Illustration of the state difficulty in the 9x9 Go. The color shows the policy output by the neural network. Purple through bright green ranges from the lower to the higher probability. }
    \label{fig:difficulty_example}
\end{figure}

==> broaderImpact.tex <==
\begin{comment}
a) who may benefit from this research,
b) who may be put at disadvantage from this research,
c) what are the consequences of failure of the system,
and d) whether the task/method leverages biases in the data.
If authors believe this is not applicable to them, authors can simply state this.
\end{comment}

Resource allocation problem usually relies on combining domain knowledge or using MCTS search in the past. In this paper, we proposed to control the simulation count by predicting difficulty score from Deep Convolutional Neural Networks.
Our method can be easily applied to many other games with MCTS and AlphaZero algorithm, such as Go, chess, shogi, and atari games. Other researchers or game designers who are limited by the computing resource problems can benefit from our proposed method and save a hung amount of time. 
By reducing the MCTS simulation counts, our algorithm can also save the energy consumption of many game-AI agents.
%Our method may fail if using inappropriate threshold to classify whether to search or not. This will cause the MCTS to stop the search early in the state that requires more simulations and make the program weaker. However, in our experiments, we can speed up about 2.5 times even using a strict threshold $thr=0.05$.

==> experiment/mp_dnn_comparison.tex <==
\begin{figure}[h]
  \centering
  \input{experiment/astw_1}
  \captionof{figure}{The results of using the PV-NN and State-UN.}
  \label{fig:stop_at_beginning}
\end{figure}

